Weaving Context Across Images: Improving Vision-Language Models through Focus-Centric Visual Chains

Vision-language models (VLMs) achieve remarkable success in single-image tasks. However, real-world scenarios often involve intricate multi-image inputs, leading to a notable performance decline as models struggle to disentangle critical information scattered across complex visual features. In this work, we propose Focus-Centric Visual Chain, a novel paradigm that enhances VLMs'perception, comprehension, and reasoning abilities in multi-image scenarios. To facilitate this paradigm, we propose Focus-Centric Data Synthesis, a scalable bottom-up approach for synthesizing high-quality data with elaborate reasoning paths. Through this approach, We construct VISC-150K, a large-scale dataset with reasoning data in the form of Focus-Centric Visual Chain, specifically designed for multi-image tasks. Experimental results on seven multi-image benchmarks demonstrate that our method achieves average performance gains of 3.16% and 2.24% across two distinct model architectures, without compromising the general vision-language capabilities. our study represents a significant step toward more robust and capable vision-language systems that can handle complex visual scenarios.

==> tables/evaluation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}llll@{}}
\toprule
Final Answer Accuracy & Subquestion Answer Accuracy & Focus Accuracy & Overall Accuracy \\ \midrule
    98                     &         95                             &      100             &       95           \\ \bottomrule
\end{tabular}%
}
\caption{Manual evaluation produced three metrics: final answer accuracy (the ratio of correct final answers), subquestion answer accuracy (the ratio of correct subquestion answers), and focus accuracy (the accuracy of the visual information attended during reasoning). Overall accuracy is the proportion of samples with all three correct. The results are weighted averages from four evaluators.}
\end{table}
